Relations between Abs-Normal NLPs and MPCCs. Part 1: Strong Constraint Qualifications

This work is part of an ongoing effort of comparing non-smooth optimization problems in abs-normal form to MPCCs. We study the general abs-normal NLP with equality and inequality constraints in relation to an equivalent MPCC reformulation. We show that kink qualifications and MPCC constraint qualifications of linear independence type and Mangasarian-Fromovitz type are equivalent. Then we consider strong stationarity concepts with first and second order optimality conditions, which again turn out to be equivalent for the two problem classes. Throughout we also consider specific slack reformulations suggested in [9], which preserve constraint qualifications of linear independence type but not of Mangasarian-Fromovitz type.

==> math-std.tex <==
% Standard math definitions -- requires amsmath

\newcommand\const{\textup{const}}
\newcommand\qtext{\quad\textup}
\newcommand\textq[1]{\text{#1}\quad}
\newcommand\qtextq{\quad\textq}
\newcommand\st{\textup{s.t.}}
\newcommand\stq{\st\quad}
\newcommand\qst{\quad\st}
\newcommand\qstq{\qst\quad}

\makeatletter
\newcommand\fcdot{\,\cdot\,}
\newcommand\fcarg[1]{\def\fc@rg{#1}\ifx\fc@rg\empty\fcdot\else\fc@rg\fi}
\makeatother
\newcommand\abs[1]{\lvert\fcarg{#1}\rvert}
\newcommand\Abs[1]{\left\lvert#1\right\rvert}
\newcommand\fracabs[2]{\frac{\abs{#1}}{\abs{#2}}}
\newcommand\fracAbs[2]{\frac{\Abs{#1}}{\Abs{#2}}}
\newcommand\absfrac\fracabs
\newcommand\Absfrac\fracAbs
\newcommand\bndint[3]{#3|_{#1}^{#2}}
\newcommand\Bndint[3]{\left.#3\right|_{#1}^{#2}}
\newcommand\bndintbr[3]{[#3]_{#1}^{#2}}
\newcommand\Bndintbr[3]{\left[#3\right]_{#1}^{#2}}
\newcommand\card\abs
\newcommand\Card\Abs
\newcommand\ceil[1]{\lceil\fcarg{#1}\rceil}
\newcommand\Ceil[1]{\left\lceil#1\right\rceil}
\newcommand\defsep\colon% alternative: \mid
\newcommand\defset[3][\defsep]{\set{#2#1#3}}
\newcommand\Defset[3][\defsep]{\Set{#2#1#3}}
\newcommand\dparlong[2]{\frac{\partial#2}{\partial#1}}% after 2010-11-08
\newcommand\dparshort[2]{\partial_{#1}#2}
\newcommand\dparlongold[2]{\frac{\partial#1}{\partial#2}}% till 2010-11-08
\newcommand\dparshortold[2]{\partial_{#2}#1}
\newcommand\dpar\dparlong
\newcommand\EEmult\cdot% alternative: \times
\newcommand\EE[1][\EEmult]{#1 10^}
\newcommand\floor[1]{\lfloor\fcarg{#1}\rfloor}
\newcommand\Floor[1]{\left\lfloor#1\right\rfloor}
\newcommand\Inv[1]{#1^{-1}}
\newcommand\HInv[1]{#1\ihr}% hermitian inverse
\newcommand\TInv[1]{#1\itp}% transpose inverse
\newcommand\norm[2][]{\lVert\fcarg{#2}\rVert\optsb{#1}}
\newcommand\Norm[2][]{\left\lVert#2\right\rVert\optsb{#1}}
\newcommand\fracnorm[3][]{\frac{\norm[#1]{#2}}{\norm[#1]{#3}}}
\newcommand\fracNorm[3][]{\frac{\Norm[#1]{#2}}{\Norm[#1]{#3}}}
\newcommand\normfrac\fracnorm
\newcommand\Normfrac\fracNorm
\newcommand\onehalf{\recip2}
\newcommand\pfrac\dparlong% synonym
\newcommand\recip{\frac1}
\newcommand\set[1]{\{#1\}}
\newcommand\Set[1]{\left\{#1\right\}}
\newcommand\snorm[2][]{\lvert\!\lvert\!\lvert
  \fcarg{#2}\rvert\!\rvert\!\rvert\optsb{#1}}
\newcommand\Snorm[2][]{\left\lvert\!\left\lvert\!\left\lvert
  #2\right\rvert\!\right\rvert\!\right\rvert\optsb{#1}}
\newcommand\sprod[3][]{\langle\fcarg{#2},\fcarg{#3}\rangle\optsb{#1}}
\newcommand\Sprod[3][]{\left\langle#2,#3\right\rangle\optsb{#1}}

\newcommand\tdpar[2]{\partial#1/\partial#2}
\newcommand\tonehalf{\trecip2}
\newcommand\hrchar{H}
\newcommand\tpchar{T}
\newcommand\hr{^\hrchar}% hermitian transpose
\newcommand\tp{^\tpchar}
\newcommand\ihr{^{-\hrchar}}
\newcommand\itp{^{-\tpchar}}
\newcommand\tadj[1]{\mskip#1\thinmuskip}% adjust space
\newcommand\hra[1][0]{^{\tadj{#1}\hrchar}}
\newcommand\tpa[1][0]{^{\tadj{#1}\tpchar}}
\newcommand\ihra[1][0]{^{\tadj{#1}{-}\hrchar}}
\newcommand\itpa[1][0]{^{\tadj{#1}{-}\tpchar}}
\newcommand\tpfrac\tdpar% synonym
\newcommand\trecip{\tfrac1}
\newcommand\without{\setminus\set}
\newcommand\Without{\setminus\Set}

\newcommand\lbound{-}
\newcommand\ubound{+}
\newcommand\splb{^{\lbound}}
\newcommand\spub{^{\ubound}}
\newcommand\sblb{_{\lbound}}
\newcommand\sbub{_{\ubound}}
\newcommand\bounds[1]{\ensuremath{[#1\splb,#1\spub]}}
\newcommand\Bounds[1]{\ensuremath{\left[#1\splb,#1\spub\right]}}

\newcommand\Strut{\rule[2.5555ex]{0pt}{0pt}}% ~1.1em
%\newcommand\Hline{\hline\Strut}   % --ck for gOMS2e

\newcommand\optsb[1]{\ifx#1\empty\else_{#1}\fi}
\newcommand\optsp[1]{\ifx#1\empty\else^{#1}\fi}
\newcommand\optindex[1]{\ifx#1\empty\else,#1\fi}
\newcommand\optmathsb\optsb
\newcommand\optmathsp\optsp
\newcommand\opttextsb[1]{\optsb{\textup{#1}}}
\newcommand\opttextsp[1]{\optsp{\textup{#1}}}
\newcommand\optmathindex\optindex
\newcommand\opttextindex[1]{\optindex{\textup{#1}}}

%% neighbourhood (by Martin Schmidt)
\newcommand{\neighbourhood}{\mathcal{N}}
\newcommand{\nh}{\neighbourhood}

%% continuous functions (by Martin Schmidt)
\newcommand{\continuousFunctions}[1]{\mathcal{C}\optsp{#1}}
\newcommand{\contFuncs}{\continuousFunctions}
\newcommand{\piecewiseContinuousFunctions}[1]{\mathcal{C}_p\optsp{#1}}
\newcommand{\pwContFuncs}{\piecewiseContinuousFunctions}

\newcommand\define{\mathrel{{\mathop:}{=}}}
\newcommand\enifed{\mathrel{{=}{\mathop:}}}


==> math-symbols.tex <==
% Math symbols -- requires amsmath

% Redefine some macros in math mode. Keep text mode definitions.
\let\TeXbar\_   % underscore -> \bar
\let\TeXhat\^   % undefined  -> \hat
\let\TeXtilde\~ % undefined  -> \tilde
\let\TeXcolon\: % \tmspace+\medmuskip{.2222em} -> \colon
\makeatletter
\newcommand\mcs@cc[3]{\leavevmode\ifmmode#1{#3}\else#2{#3}\fi}
\renewcommand\_{\mcs@cc\bar\TeXbar}
\renewcommand\^{\mcs@cc\hat\TeXhat}
\renewcommand\~{\mcs@cc\tilde\TeXtilde}
\renewcommand\:{\mcs@cc\colon\TeXcolon\relax}
\makeatother
\PackageInfo{math-symbols}{Redefining
 \string\_, \string\^, \string\~, \string\: in math mode.
 \MessageBreak Keeping text mode definitions.
 \MessageBreak Saving original commands as \string\TeXbar, \string\TeXhat,
 \MessageBreak \string\TeXtilde, \string\TeXcolon}

\newcommand\0\emptyset
\newcommand\bigM{M}
\newcommand\bigO{O}
\newcommand\smallo{o}
\newcommand\oo\infty
\newcommand\ox\otimes
\ifnum\FmtChoice=0
% Redefine unuesed gOMS2e macro: \x=macro: @{\extracolsep{\fill}}.
\renewcommand\x\times
\else
\newcommand\x\times
\fi

\newcommand\itxt{\textup}% text in math indices
\newcommand\tsb[1]{_{\itxt{#1}}}% text subindex
\newcommand\tsp[1]{^{\itxt{#1}}}% text superindex

\newcommand\boundary\partial
\newcommand\cond\kappa
\newcommand\condabs{\cond\tsb{abs}}\newcommand\abscond\condabs
\newcommand\condrel{\cond\tsb{rel}}\newcommand\relcond\condrel
\newcommand\convrad\rho
\newcommand\eps\epsilon
\newcommand\veps\varepsilon
\newcommand\epsmach{\veps\tsb{M}}
\newcommand\specrad\rho
\newcommand\spectrum\sigma
\newcommand\uvec{\mathbf1}

% Some arrows.
\newcommand\larrow\leftarrow
\newcommand\rarrow\to% \rightarrow
\newcommand\lrarrow\leftrightarrow
\newcommand\Larrow\longleftarrow
\newcommand\Rarrow\longrightarrow
\newcommand\LRarrow\longleftrightarrow
\newcommand\xlarrow\xleftarrow
\newcommand\xrarrow\xrightarrow
\newcommand\lArrow\Leftarrow
\newcommand\rArrow\Rightarrow

% Right-shifted relation symbols for alignment with :=
\newcommand\crel[1]{\mathrel{\hphantom:{#1}}}
\newcommand\isom{\crel\cong}
\newcommand\eqls{\crel=}

